TEEMon: A continuous performance monitoring framework for TEEs

Trusted Execution Environments (TEEs), such as Intel Software Guard eXtensions (SGX), are considered as a promising approach to resolve security challenges in clouds. TEEs protect the confidentiality and integrity of application code and data even against privileged attackers with root and physical access by providing an isolated secure memory area, i.e., enclaves. The security guarantees are provided by the CPU, thus even if system software is compromised, the attacker can never access the enclave's content. While this approach ensures strong security guarantees for applications, it also introduces a considerable runtime overhead in part by the limited availability of protected memory (enclave page cache). Currently, only a limited number of performance measurement tools for TEE-based applications exist and none offer performance monitoring and analysis during runtime. This paper presents TEEMon, the first continuous performance monitoring and analysis tool for TEE-based applications. TEEMon provides not only fine-grained performance metrics during runtime, but also assists the analysis of identifying causes of performance bottlenecks, e.g., excessive system calls. Our approach smoothly integrates with existing open-source tools (e.g., Prometheus or Grafana) towards a holistic monitoring solution, particularly optimized for systems deployed through Docker containers or Kubernetes and offers several dedicated metrics and visualizations. Our evaluation shows that TEEMon's overhead ranges from 5% to 17%.

==> sgx_driver_hooks.tex <==
%!TEX root = ./paper.tex

\begin{table}[t!]
    % \scriptsize
    \caption{Exported SGX driver hooks.\robert{Not done yet.}\vspace{-5pt}}\label{tab:dirverhooks}
    \small
    \setlength{\tabcolsep}{3pt}
    \renewcommand\theadfont{\bfseries}
    \centering
    \begin{tabular}{c>{\centering\arraybackslash}p{0.6\columnwidth}}
      \rowcolor{gray!25}
      \textbf{Name} & \textbf{Content}\\
      \hline
      sgx\_nr\_total\_epc\_pages & \# of EPC pages reserved \\
      sgx\_nr\_free\_pages & \# of currently free EPC pages \\
      sgx\_nr\_low\_pages & min. \# of EPC pages before swapping \\
      sgx\_nr\_high\_pages & \# of free EPC pages w/o swapping \\
      sgx\_nr\_marked\_old & \# of EPC pages marked as old \\
      sgx\_nr\_evicted & \# of EPC pages that were evicted \\
      sgx\_nr\_alloc\_pages & \# of EPC pages pulled back after evict. \\
      sgx\_nr\_enclaves & \# of Enclaves currently running \\
      sgx\_nr\_reclaimed & \# of EPC pages that were reclaimed \\
      sgx\_nr\_added\_pages & \# of EPC pages added to enclaves \\
      sgx\_init\_enclaves & \# of enclaves initialized \\
      sgx\_loaded\_back & \# of EPC pages loaded from memory \\
      \hline
    \end{tabular}
    %\spaceafterfloat
    %\vspace{-10pt}
    \end{table}
    

==> space-tricks.tex <==
% -*- root: main.tex -*-

%space left between floats.
\setlength{\floatsep}{4mm}
% space between last top float or first bottom float and the text.
\setlength{\textfloatsep}{2mm}

% space left on top and bottom of an in-text float.
\setlength{\intextsep}{0.5mm}


% This has the largest impact:
% space above caption
\setlength{\abovecaptionskip}{9pt}


%space below caption
\setlength{\belowcaptionskip}{0mm}

%% Change figure handling
\renewcommand{\topfraction}{0.9}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{1}



\usepackage[inline]{enumitem}
\setlist{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}

%\usepackage[subtle]{savetrees}
% \usepackage[moderate]{savetrees}

\usepackage{setspace}
\usepackage[margin=5pt,font={stretch=0.9}]{caption}
%\usepackage[margin=8pt,font={small,bf,stretch=0.85}]{caption}


%\usepackage[small,compact,noindentafter]{titlesec}
%\usepackage[compact]{titlesec}
%
%\titlespacing\section{0pt}{6pt plus 2pt minus 2pt}{2pt plus 2pt minus 2pt}
%\titlespacing\subsection{0pt}{4pt plus 2pt minus 2pt}{2pt plus 1pt minus 1pt}
%\titlespacing{\paragraph}{0pt}{2pt plus 0pt minus 1pt}{1.0ex}
%

